Finding Average Regret Ratio Minimizing Set in Database

Selecting a certain number of data points (or records) from a database which "best" satisfy users' expectations is a very prevalent problem with many applications. One application is a hotel booking website showing a certain number of hotels on a single page. However, this problem is very challenging since the selected points should "collectively" satisfy the expectation of all users. Showing a certain number of data points to a single user could decrease the satisfaction of a user because the user may not be able to see his/her favorite point which could be found in the original database. In this paper, we would like to find a set of k points such that on average, the satisfaction (ratio) of a user is maximized. This problem takes into account the probability distribution of the users and considers the satisfaction (ratio) of all users, which is more reasonable in practice, compared with the existing studies that only consider the worst-case satisfaction (ratio) of the users, which may not reflect the whole population and is not useful in some applications. Motivated by this, in this paper, we propose algorithms for this problem. Finally, we conducted experiments to show the effectiveness and the efficiency of the algorithms.

==> improvement.tex <==



\subsubsection{Strategies for Improvement}
\label{subsubsec:alg:improvement}

Now, we put all the ideas discussed before together to give the final algorithm. Note that in the following procedure, there is no assumption on the distribution of the utility functions. That is, any distribution can be handled using this process. The final process is done in the following steps:

\begin{itemize}
\item Construct an R*-tree \cite{R*} from the $n$ points in the database.
\item If the distribution of the utility functions is not discrete, do the sampling based on the Section \ref{sec:sample}. It will result in a set $F_N$ of $N$ utiluty functions.
\item For each sample or existing utility function (if their distribution is discrete), calculate $\max_{p\in D}f(p)$. While calculating this, keep track of the best point for each user as well as for each point, the users for whom the point is the best point. Besides, in two separate arrays store $\max_{p\in D}f(p)$ and $\max_{p\in S}f(p)$, which will be equal initially.
\item Use Algorithm $\ref{algo}$ to find the solution set. For the calculation of the average regret ratio, use the process explained in Section 5.3.
\end{itemize}


First, we construct an R*-tree from the $n$ points we have in the database $D$ and initialize $S$ to $D$. Then, if the distribution of the utility function is not discrete, we need to perform the sampling. We determine the sample size, $N$, from the two user given parameters $\epsilon$ and $\sigma$. We draw a sample of size $N$, $F_N$, based on the probabilities given in $\eta(.)$.

After that, we go through all the $N$ users to find the best point of each user in $S$, which is equal to $D$. We keep track of the best point for each user in $S$, and for each point in $S$, the users who find that point the best in $S$. For finding the best point for a user, we compare its utility function with the utility function of the privious user for whom the best point is known. Then, we define a query rectangle based on the weight differences and the best point of the pious user and search for the current user's best point in the R*-tree, as discussed in Section 5.3.

Next, we start a loop and for $n - k$ iterations and at each iteration find the point whose removal affects the average regret ratio the least. To do so, at each iteration $i$, $1 \leq i \leq n - k$ we go through the points whose $arr(S_{i - 1} - \{p\})$ is lower than $arr(S_{i} - \{p'\})$ where $p'$ is the $(k + 1)$-th lowest point, $S_{i}$ is the solution set at the $i$-th iteration ($S_{0} = S_{1} = D$) and the points are sorted based on $arr(S_{i - 1} - \{p\})$ values. For each point, we remove it from $S$, calculate average regret ratio and then select the point after whose removal, average regret ratio is the lowest. While calculating the average regret ratio, we only go through the database to look for a user's best point if the best point that we had stored for the user has been already removed from the solution set. Otherwise, we just use the stored value. Moreover, in calculation of the average regret ratio, whe only go through the users who have been affected by the removal of the last points. After the $n - k$ iterations, we return the set $S$. The correctness of this procedure, as well as the bounds on its error, follows from the next theorem.

\begin{theorem} Let $D$ be a set of points, $F$ a set of the utility functions with the probability distribution $\Theta$ and $k$ the number of desired representative points from the database.
\begin{itemize}
\item If $\Theta$ is a discrete distribution and the set of utility functions is finite, then Algorithm $\ref{algo}$ returns a set, $S$, of $k$ points for which $arr(S) \leq \frac{e^t - 1}{t}arr(S_O)$, where $S_O$ is a set of $k$ points with the lowest possible average regret ratio, i.e. the optimal solution.
\item Otherwise, the sampling of the utility functions based on the error and confidence parameters $\epsilon$ and $\sigma$ and running Algorithm $\ref{algo}$ results in the solution set  $S$, for which $arr^*(S) < \frac{e^t - 1}{t}(arr^*(S_O) + \epsilon) + \epsilon$ with the confidence of 1 - $\sigma$, where $arr^*(S)$ is the true value of the average regret ratio (not the value calculated by sampling).
\end{itemize}
\label{thm:discreteDistribution}
\end{theorem}



To illustrate the use of theorem 6, consider the following situations based on the data given in Tables 1 and 2 and $k = 2$. Then, the set $F$ is a finite set, consisting of 4 users, namely Alex, Jerry, Tom and Sam, and each user has the probability 0.25. Then, as the distribution of the users is discrete and there are finite number of users, then we use the Algorithm $\ref{algo}$ and return the result $S = $\{Holiday Inn, Intercontinental\} as explained in Section 5.2. We can also solve this problem by sampling. We need to choose a sample size $N$ and sample a finite number of utility functions from based on the probability distribution of the utility functions in the set $F$ and put them in the set $F_N$. Then, we can use the Algorithm $\ref{algo}$ to return the final solution set $S$. For instance, the sampled set may be $F_N = $ \{Alex, Alex, Sam, Tom, Alex, Tom, Jerry, Jerry, Sam, Sam\}. Then, the algorithm will first set  $S = $\{Holiday Inn, Shangri la, Intercontinental, hilton\}. Then it calculates $arr(S - $\{Holiday Inn\}$) = 0.0134$, $arr(S - $\{Shangri la\}$) = 0.00313$, $arr(S - $\{Intercontinental\}$) = 0.0336$ and $arr(S - $\{Hilton\}$) =  0.0960$. Then it sets $S = S - $\{Shangri la\}, as removal of Shangri la results in the least increase in the average regret ratio (average regret ratio is 0 initially, with $S = D$). In the second iteration, the algorithm calculates  $arr(S - $\{Holiday Inn\}$) = 0.125$, $arr(S - $ \{Intercontinental\}) $= 0.0368$ and $arr(S - $\{Hilton\}$) = 0.0991$. Then, the algorithm sets $S = S - $\{Intercontinental\}. Since now the size of $S$ is equal to $k$, the algorithm returns $S = $\{Holiday Inn, Hilton\} as the final solution with $arr(S) =  0.0368$.

To see how the final algorithm works, consider the following example. Let $D$ and $F$ be the data given in Tables 1 and 2. Additionally, assume that $N$, the sampling size is 10. So, the algorithm first choses 10 points randomly from $F$, assuming a uniform distribution of the utility functions, and puts them in the set $F_N$. Then, it constructs an R*-tree from the 4 points in $D$ and sets $S$ to be equal to $D$. After that, it goes through all the 10 utility functions and finds their best point in $S$ and also calculates $sat(S, f) = sat(D, f)$ for each utility function, $f$. Then we start a loop and at each iteration, for (some of) the points $s \in S$ we remove $s$ from $S$, calculate the average regret ratio based on the explained method, and add $s$ back to $S$. Then, we find the minimum of all the calculated average regret ratios and let $S$ to be the argmax of that value. This way, the size of $S$ is reduced by one. We continue untill the size of $S$ is equal to $k = 1$ and then return $S$ as the solution.


